Two-loop QED/QCD corrections for polarized $\gamma\gamma\rightarrow\gamma\gamma$ process in SANCphot

The new version of the SANCphot integrator has been prepared for fast and stable numerical calculations up to two loops for polarized light-by-light scattering. One-loop modules based on the helicity formalism with massive particles and two-loop modules with massless particles inside the loops are used. The presented study is driven by the potential of polarized photon beams to probe the high energy region. This study is a contribution to the research program of the CEPC project being under development in China.

==> latex-defs.tex <==
% latex definitions

\newcommand{\nll}{\nonumber\\}
\newcommand{\mr}[1]{\mathrm{#1}}
\newcommand{\alem}{\alpha_{em}}
\newcommand{\alsS}{\alpha^2_{_S}}
\newcommand{\sss}[1]{\scriptscriptstyle{#1}}
\newcommand{\sew}{\sin^2 \theta_{\mr{eff}}^{\mr{lept}}}
%----------------------------    chi2 ...
\def\c2{\chi^2}
\def\cndf{\chi^2/\mr{n.d.f.}}

%---------------------------  processes 




\def\gggg{\gamma\gamma\rightarrow\gamma\gamma}



\def\L{ {\cal L }}
\def\O{ {\cal O }}
\def\C{ {\cal C }}
\def\D{ {\cal D }}
\def\R{ {\cal R }}








